RegBN: Batch Normalization of Multimodal Data with Regularization

Recent years have witnessed a surge of interest in integrating high-dimensional data captured by multisource sensors, driven by the impressive success of neural networks in the integration of multimodal data. However, the integration of heterogeneous multimodal data poses a significant challenge, as confounding effects and dependencies among such heterogeneous data sources introduce unwanted variability and bias, leading to suboptimal performance of multimodal models. Therefore, it becomes crucial to normalize the low- or high-level features extracted from data modalities before their fusion takes place. This paper introduces a novel approach for the normalization of multimodal data, called RegBN, that incorporates regularization. RegBN uses the Frobenius norm as a regularizer term to address the side effects of confounders and underlying dependencies among different data sources. The proposed method generalizes well across multiple modalities and eliminates the need for learnable parameters, simplifying training and inference. We validate the effectiveness of RegBN on eight databases from five research areas, encompassing diverse modalities such as language, audio, image, video, depth, tabular, and 3D MRI. The proposed method demonstrates broad applicability across different architectures such as multilayer perceptrons, convolutional neural networks, and vision transformers, enabling effective normalization of both low- and high-level features in multimodal neural networks. RegBN is available at \url{https://github.com/mogvision/regbn}.

==> oldVersion/SomeNotesFutureWork.tex <==

% latest relevant papers
% https://arxiv.org/pdf/2305.11443.pdf
% baseline > https://openaccess.thecvf.com/content/CVPR2023/papers/Yi_A_Simple_Framework_for_Text-Supervised_Semantic_Segmentation_CVPR_2023_paper.pdf

% check this 
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8918259&casa_token=FFdM1cRHlssAAAAA:1jqeNpK6w7rjGjPBkyKWZ5npIyDLRgtEbGKfDhuMgYuQRr_UcYye3lLTo0vlFTrE6EA125Po

% suggestions (after submission):
% 1- https://arxiv.org/pdf/2307.08927.pdf as another baseline tech (robotics)
% 2- https://irvlutd.github.io/Proto-CLIP/ 


% TODO: 
%1 Minor Comment: Ambiguous notations: In line 101 and 102, what is the meaning of N and M? Authors' Response:  We appreciate the reviewer for highlighting this point. In this study,  'f' and 'g’ are N- and M-dimensional feature maps, respectively. We will make the necessary revision to the text to accurately reflect this.

% 2>>> RegBN: Regularized Batch Normalization (RegBN)
% >>>>>>>>>>>>>>>>>>> Replace Appendix with Suppl (big mistake!!!)






\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.



\section{Supplementary Material}

Authors may wish to optionally include extra information (complete proofs, additional experiments and plots) in the appendix. All such materials should be part of the supplemental material (submitted separately) and should NOT be included in the main submission.




\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}



\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2023/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}





tsNE:
    image([448, 160]) audio([448, 320]) norm and concat ([448, 480]) concat plus mlp([448, 64]) torch.Size([448])
ours     105560 98       99.10714285714286
mdn      156760 97.54    98.68392857142857
identity 105560 97.23    98.4375
trains nums:  1050
test num: 450
AV-MNIST



Multibench >> table 24 << running time, memory, etc


\item ??? address this: prof. Christian: do you want to add that it does not introduce more parameters???? say that: unlike the conventional bns that normalise along the model's objective, Regbn uses its own trainable parameters???? 





cite these paper in the future:
https://openaccess.thecvf.com/content/CVPR2022/papers/Bohle_B-Cos_Networks_Alignment_Is_All_We_Need_for_Interpretability_CVPR_2022_paper.pdf

https://openreview.net/pdf?id=6ve2CkeQe5S



==> rebuttal.tex <==


\pagebreak



\begin{table}
  \caption*{\textbf{[Updated Table I.7 with LN results]} Training cross-entropy (CE) loss,   test accuracy (ACC), and test balanced accuracy (BA) on the ADNI dataset~\cite{jack2008alzheimer}. Baseline is a combination of techniques developed in~\cite{hager2023best,wolf2022daft}. 
  }
  \centering
  \begin{tabular}{@{\extracolsep{4pt}}lcccc@{}}
    \toprule
     Method  &Norm. params. & Training CE  & \multicolumn{2}{c}{Test}  \\
    \cmidrule{4-5} %\addlinespace
    & ($\#$) &loss$\downarrow$ & ACC (\%) $\uparrow$ & BA (\%)$\uparrow$ \\ 
    \midrule
    BN    & 512 &  0.641±0.01  &  48.8±4.4 & 48.3±4.5\\
    GN    & 512 &  0.649±0.01  &  48.4±4.6 & 47.9±4.5\\
    LN    & 512 &  0.646±0.01  &  48.5±4.4 & 48.1±4.5\\
    IN    & 512 &  0.647±0.01  &  48.2±4.5 & 48.0±4.4\\
    MDN   & 0   &  0.619±0.03  & 50.4±4.8 & 50.1±5.6 \\
    PMDN  & 4,096 & 0.632±0.03 & 49.7±6.2 & 49.6±7.5 \\
    RegBN & 0 & {0.596±0.01} & {53.0±3.1} & {52.3±3.7} \\
    \bottomrule
  \end{tabular}
\end{table}



\begin{table}
  \caption*{\textbf{[Updated Table I.9 with LN results]} Accuracy of classification results on the synthetic dataset in the presence of a confounder. Comparison of the reference to an approach without (W/O) normalization and several normalization techniques. Due to randomness, we reported the mean and std of results over 100 runs.}
  \centering
  \begin{tabular}{@{\extracolsep{4pt}}l cc cccc@{}}
    \toprule
    Normalization   &\multicolumn{2}{c}{Norm. params. ($\#$)}   & \multicolumn{2}{c}{Experiment I} & \multicolumn{2}{c}{Experiment II}  \\
    \cmidrule{2-3} \cmidrule{4-5}  \cmidrule{6-7} %\addlinespace
    Method &  MLP & CNN & MLP & CNN & MLP & CN \\
    \midrule
    \emph{reference} &      - &   -      & \emph{87.5}  & \emph{87.5}  & \emph{75.0} & \emph{75.0}\\
    W/O normalization  &  0  &  0  & 96.2±0.4 & 96.3±0.3 & 86.7±0.6 & 85.4±0.7\\
    BN         & 256 & 112 & 96.4±0.4 & 94.9±0.2 & 83.1±0.8 & 85.2±0.3\\
    GN         & 256 & 112  & 96.3±0.3 & 95.7±0.3 & 84.6±0.6 & 86.7±0.4\\
    LN         & 256 &  112 & 96.1±0.3 & 95.8±0.2 & 85.1±0.5& 84.7±0.3\\
    IN         & 256 & 112  & 96.4±0.4 & 95.9±0.2 & 84.6±0.4 & 83.2±0.9 \\
    MDN   &   0   &   0       & 91.9±0.7 & 89.7±0.7 & 79.1±0.6  & 82.2±0.7\\
    PMDN  &  2048 &   201,728 & 93.4±0.6 & 92.7±0.5 & 80.8±0.7  & 84.3±0.8\\
    RegBN &   0   &   0       & 87.3±0.9 & 88.2±0.8 & 76.2±0.8  & 76.8±0.9\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure*}
\centering
    \includegraphics[width=1.05\textwidth]{suppl/screen.png}
\caption*{Figure 1. Training (LOSS) and validation results on Colored-and-gray MNIST. The results of the baseline method, PMR, are shown in blue, and those of PMR+RegBN in orange. }
\end{figure*}
